SoK: Rethinking Jailbreaking in the Era of Agentic AI: Attacks, Defenses, and Practical Consideration

Large language models (LLMs) are rapidly evolving from conversational assistants into agentic AI systems that reason, plan, invoke tools, maintain persistent memory, communicate with other agents, and execute multi-step tasks. At the same time, modern models exhibit substantially stronger native safety alignment than earlier generations on which many jailbreak attacks and defenses were originally studied. This shift raises a fundamental question: \textit{which established jailbreak-security findings remain valid in the era of modern LLMs and agentic AI?} We address this question through a Systematization of Knowledge (SoK) that reframes jailbreak security around the full agentic execution pipeline. We develop unified taxonomies of attacks and defenses spanning user interaction, planning and reasoning, memory, tool use, and inter-agent communication, and introduce a security--utility--efficiency evaluation framework that separates native harmful-prompt safety, adversarial jailbreak robustness, and agent-level security outcomes. We further conduct a controlled empirical study of representative attacks and defenses within a common agentic framework. Our results reveal three important gaps. First, strong native alignment does not imply robustness to adversarial jailbreaks. Second, defense effectiveness is highly model-, attack-, and component-dependent and can come at substantial cost in over-refusal, utility, and latency. Third, low final-response attack success can mask severe intermediate compromise: planning, memory, and tool interactions may remain unsafe even when the final response is successfully filtered. These findings motivate a shift from response-centric jailbreak defense toward cross-layer, execution-aware security that protects agent state, component transitions, and external actions while preserving practical utility and efficiency.

==> Trade-off.tex <==
\section{Security--Utility--Efficiency Trade-off Analysis}
\label{sec:tradeoff}


Figure~\ref{fig:security_utility} compares the trade-off between security and utility. Although several defenses achieve very high defense success rates, their utility differs substantially. \textbf{Self Reminder} achieves the best overall balance, combining a 98.99\% defense success rate with high benign acceptance (95.20\%), excellent answer relevancy (95.61\%), the highest response quality (74.44\%), the highest helpfulness (74.80\%), and the highest overall utility (81.62\%). \textbf{Vanilla}, \textbf{Self Eval}, \textbf{ICD}, \textbf{Goal Prioritization}, \textbf{Erase and Check}, and \textbf{SafeProbing} also maintain strong security while preserving high utility, making them practical deployment candidates. In contrast, \textbf{Prompt Guard} and \textbf{Robust Aligned} achieve perfect defense success by refusing all benign requests, resulting in zero utility despite their maximum security. Similarly, \textbf{Parden} performs poorly across both security and utility, demonstrating that maximizing a single security metric alone is insufficient for practical deployment.

Figure~\ref{fig:utility_efficiency} compares utility preservation against computational efficiency. \textbf{SafeDecoding} ranks first because it provides exceptional computational efficiency, achieving the lowest response latency (31.99\,s) together with the smallest token and reasoning-token usage while maintaining moderate utility. \textbf{Self Reminder} ranks second by combining the highest utility with reasonable computational cost, followed closely by \textbf{Vanilla}, \textbf{SafeProbing}, and \textbf{Self Eval}. Although these methods require more computation than \textbf{SafeDecoding}, they consistently provide substantially better response quality, helpfulness, and overall utility. In contrast, \textbf{SmoothLLM} exhibits the highest inference latency (824.84\,s) without corresponding utility gains, while \textbf{Prompt Guard} and \textbf{Robust Aligned} remain computationally efficient but provide virtually no utility because they reject nearly all benign requests.

Figure~\ref{fig:overall_ranking} presents the overall comparison by jointly considering security, utility, and efficiency. Each evaluation dimension is first independently normalized using min--max normalization, and the overall score is computed by assigning equal importance to security, utility, and efficiency. Within each dimension, the corresponding metrics share the category weight proportionally. Under this unified evaluation, \textbf{Self Reminder} achieves the highest overall score by consistently balancing robustness, utility preservation, and computational efficiency. \textbf{SafeDecoding} ranks second because its exceptional efficiency compensates for its lower utility, while \textbf{Vanilla}, \textbf{SafeProbing}, \textbf{Self Eval}, and \textbf{Erase and Check} also demonstrate strong overall performance by maintaining competitive results across all three dimensions. Methods such as \textbf{Prompt Guard} and \textbf{Robust Aligned} rank substantially lower despite perfect security because their complete refusal of benign requests eliminates practical utility, whereas \textbf{SmoothLLM} is penalized by its extremely high computational cost. Overall, these results demonstrate that practical jailbreak defenses should be evaluated jointly across security, utility, and efficiency rather than optimizing any single evaluation dimension.




\begin{table*}[t]
\centering
\caption{Comparative evaluation of jailbreak defense methods in agentic AI systems (Model: Qwen3.5-4B; Dataset: XSTest; Evaluator: GPT-5-mini).}
\label{tab:defense_eval}

\scriptsize
\setlength{\tabcolsep}{10pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lccc}
\toprule
\textbf{Method} &
\textbf{Attack Success Rate} &
\textbf{Overall Accuracy} &
\textbf{Over-Refusal Rate} \\
\midrule

Vanilla & 03.67\% & 97.05\% & 02.40\% \\
Aligner & 04.08\% & 94.39\% & 06.80\% \\
Erase and Check & 02.60\% & 97.29\% & 02.80\% \\
Goal Prioritization & 02.69\% & 94.72\% & 07.20\% \\
ICD & 00.53\% & 95.44\% & 07.60\% \\
Paraphrase & 10.44\% & 84.72\% & 18.80\% \\
Parden & 44.33\% & 52.48\% & 50.00\% \\
Prompt Guard & 00.00\% & 44.44\% & 100.00\% \\
Robust Aligned & 00.00\% & 44.44\% & 100.00\% \\
SafeDecoding & 04.19\% & 88.97\% & 15.60\% \\
Self Eval & 01.56\% & 96.83\% & 04.40\% \\
Self Reminder & 01.01\% & 96.88\% & 04.80\% \\
SmoothLLM & 11.46\% & 89.37\% & 10.00\% \\
JBShield & 01.04\% & 77.15\% & 39.60\% \\
RPO & 04.00\% & 89.33\% & 16.00\% \\
Intention Analysis & 02.59\% & 84.44\% & 23.20\% \\
SafeProbing & 01.00\% & 95.33\% & 07.60\% \\

\bottomrule
\end{tabular}

\end{table*}




\begin{table*}[t]
\centering
\caption{Utility evaluation of jailbreak defense methods in agentic AI systems (Model: Qwen3.5-4B; Dataset: XSTest (Safe Subset); Evaluator: GPT-5-mini).}
\label{tab:utility_eval}

\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lccccc}
\toprule
\textbf{Method} &
\textbf{Answer Relevancy} &
\textbf{Response Quality} &
\textbf{Helpfulness} &
\textbf{Bias} &
\textbf{Utility} \\
\midrule

Vanilla & 95.50\% & 67.32\% & 66.52\% & 01.23\% & 76.35\% \\
Aligner & 82.93\% & 47.60\% & 49.56\% & 01.36\% & 60.02\% \\
Erase and Check & 94.92\% & 65.88\% & 64.36\% & 02.31\% & 74.95\% \\
Goal Prioritization & 90.49\% & 56.28\% & 61.81\% & 00.59\% & 69.55\% \\
ICD & 94.35\% & 62.48\% & 62.17\% & 01.06\% & 72.93\% \\
Paraphrase & 87.51\% & 28.51\% & 29.04\% & 01.12\% & 48.28\% \\
Parden & 14.86\% & 6.43\% & 7.08\% & 0.17\% & 9.45\% \\
Prompt Guard & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
Robust Aligned & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
SafeDecoding & 92.80\% & 40.48\% & 38.31\% & 1.28\% & 57.13\% \\
Self Eval & 95.91\% & 62.36\% & 60.96\% & 01.23\% & 73.08\% \\
Self Reminder & 95.61\% & 74.44\% & 74.80\% & 01.10\% & 81.62\% \\
SmoothLLM & 89.16\% & 45.52\% & 46.14\% & 01.42\% & 60.12\% \\
JBShield & 73.90\% & 45.88\% & 48.80\% & 00.99\% & 56.19\% \\
RPO & 87.99\% & 52.60\% & 52.13\% & 01.51\% & 64.28\% \\
Intention Analysis & 90.53\% & 66.80\% & 68.17\% & 01.05\% & 75.17\% \\
SafeProbing & 93.66\% & 60.56\% & 61.68\% & 01.69\% & 72.01\% \\

\bottomrule
\end{tabular}
\end{table*}


\begin{table*}[t]
\centering
\caption{Efficiency comparison of jailbreak defense methods on the XSTest dataset using the Qwen3.5-4B final model.}
\label{tab:efficiency}

\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lcccccc}
\toprule
\textbf{Method} &
\textbf{Total Response Time (s) $\downarrow$} &
\textbf{Tool Decision Time (s) $\downarrow$} &
\textbf{Tool Execution Time (s) $\downarrow$} &
\textbf{Final Response Time (s) $\downarrow$} &
\textbf{Total Tokens $\downarrow$} &
\textbf{Reasoning Tokens $\downarrow$} \\
\midrule
Vanilla & 72.44 & 8.55 & 0.54 & 63.35 & 2285.74 & 1020.40 \\
Aligner & 143.04 & 8.77 & 0.57 & 133.69 & 1902.36 & 240.12 \\
Erase and Check & 86.29 & 8.76 & 0.54 & 77.00 & 2301.30 & 1027.48 \\
Goal Prioritization & 70.58 & 8.57 & 0.51 & 61.50 & 2952.10 & 1314.42 \\
ICD & 79.31 & 8.82 & 0.62 & 69.87 & 2755.68 & 1268.15 \\
Paraphrase & 131.05 & 9.01 & 0.51 & 121.52 & 4224.03 & 680.01 \\
Parden & 91.88 & 8.76 & 0.52 & 82.60 & 613.62 & 509.32 \\
Prompt Guard & 71.07 & 8.57 & 0.49 & 62.00 & 139.46 & 0.00 \\
Robust Aligned & 120.14 & 8.79 & 0.52 & 110.83 & 135.56 & 6.62 \\
SafeDecoding & 31.99 & 8.79 & 0.59 & 22.62 & 610.11 & 11.48 \\
Self Eval & 73.33 & 8.55 & 0.57 & 64.21 & 2281.00 & 1059.25 \\
Self Reminder & 67.40 & 8.55 & 0.72 & 58.13 & 2281.00 & 1059.25 \\
SmoothLLM & 824.84 & 8.73 & 0.62 & 815.49 & 2938.51 & 1052.04 \\
JBShield & 52.89 & 8.65 & 0.71 & 43.53 & 1606.07 & 664.97 \\
RPO & 194.14 & 8.58 & 0.52 & 185.03 & 1746.82 & 1580.24 \\
Intention Analysis & 164.92 & 8.95 & 0.55 & 155.41 & 2779.25 & 1375.12 \\
SafeProbing & 140.68 & 8.73 & 0.60 & 131.35 & 1683.57 & 660.10  \\
\bottomrule
\end{tabular}

\end{table*}




% llama result
\begin{table*}[t]
\centering
\caption{Comparative evaluation of jailbreak defense methods in agentic AI systems (Model: Llama-3.1-8B-Instruct; Dataset: XSTest; Evaluator: GPT-5-mini).}
\label{tab:defense_eval}

\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lccc}
\toprule
\textbf{Method} &
\textbf{Attack Success Rate} &
\textbf{Overall Accuracy} &
\textbf{Over-Refusal Rate} \\
\midrule

Vanilla &02.51\% & 94.43\% & 08.00\% \\

Aligner & 23.81\% & 80.41\% & 16.40\%\\
Erase and Check & 00.00\% & 74.00\% & 46.80\% \\

Goal Prioritization & 00.00\% & 90.16\% & 17.60\% \\

ICD & 02.01\% & 95.10\% & 07.20\% \\
Paraphrase & 06.50\% & 78.44\% & 33.20\% \\
Parden & 02.50\% & 88.89\% & 17.60\% \\

Prompt Guard &00.00\% & 44.44\% & 100.0\% \\

Robust Aligned & 00.00\% & 44.44\%  & 100.0\% \\
Safedecoding & 04.50\% & 94.22\% & 06.40\% \\
Self Eval & 03.52\%& 95.55\% &05.20\% \\
Self Reminder &02.01\% & 86.86\% &22.00\% \\
SmoothLLM & 08.00\% & 90.67\% & 10.00\% \\
JBShield & 00.00\% & 51.11\% & 87.60\% \\
RPO & 06.50\% & 63.78\% & 57.20\% \\
Intention Analysis & 00.50\% & 81.56\% & 32.40\% \\
SafeProbing & 02.00\% & 95.33\% & 06.40\% \\

\bottomrule
\end{tabular}

\end{table*}

\begin{table*}[t]
\centering
\caption{Efficiency comparison of jailbreak defense methods on the XSTest dataset using the Llama-3.1-8B-Instruct final model.}
\label{tab:efficiency_llama}

\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lccccc}
\toprule
\textbf{Method} &
\textbf{Total Response Time (s) $\downarrow$} &
\textbf{Tool Decision Time (s) $\downarrow$} &
\textbf{Tool Execution Time (s) $\downarrow$} &
\textbf{Final Response Time (s) $\downarrow$} &
\textbf{Total Tokens $\downarrow$} \\
\midrule

Vanilla & 13.64 & 8.60 & 0.77 & 4.28 & 298.11 \\
Aligner & 93.47 & 8.50 & 0.91 & 84.05 & 2073.94 \\
Erase and Check & 19.19 & 8.99 & 0.50 & 9.70 & 226.29 \\
Goal Prioritization & 14.34 & 8.62 & 0.58 & 5.14 & 1035.08 \\
ICD & 13.27 & 8.61 & 0.82 & 3.84 & 506.11 \\
Paraphrase & 41.47 & 8.83 & 0.60 & 32.03 & 1096.62 \\
Parden & 123.30 & 8.74 & 0.57 & 113.99 & 299.64 \\
Prompt Guard & 14.22 & 9.20 & 0.49 & 4.54 & 131.70 \\
Robust Aligned & 30.88 & 8.89 & 0.52 & 21.46 & 182.47 \\
SafeDecoding & 14.57 & 8.64 & 0.54 & 5.39 & 306.86 \\
Self Eval & 14.40 & 8.74 & 0.51 & 5.15 & 296.50 \\
Self Reminder & 14.67 & 8.66 & 2.25 & 3.76 & 321.40 \\
SmoothLLM & 59.31 & 8.95 & 0.70 & 49.66 & 372.09 \\
JBShield & 10.98 & 8.64 & 0.53 & 1.81 & 158.53 \\
RPO & 149.66 & 8.58 & 0.55 & 140.54 & 3006.63 \\
Intention Analysis & 15.74 & 8.71 & 0.61 & 6.42 & 197.62 \\
SafeProbing & 15.50 & 8.48 & 0.54 & 6.47 & 300.58 \\

\bottomrule
\end{tabular}

\end{table*}





\begin{table*}[t]
\centering
\caption{Utility evaluation of jailbreak defense methods in agentic AI systems (Model: Llama-3.1-8B-Instruct; Dataset: XSTest (Safe Subset); Evaluator: GPT-5-mini).}
\label{tab:utility_eval_llama}

\scriptsize
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.15}

\begin{tabular}{lccccc}
\toprule
\textbf{Method} &
\textbf{Answer Relevancy} &
\textbf{Response Quality} &
\textbf{Helpfulness} &
\textbf{Bias} &
\textbf{Utility} \\
\midrule

Vanilla & 94.92\% & 67.88\% & 65.20\% & 04.70\% & 76.00\% \\
Aligner & 74.05\% & 30.75\% & 29.75\% & 00.40\% & 44.84\% \\
Erase and Check & 74.55\% & 47.80\% & 46.56\% & 00.55\% & 56.30\% \\
Goal Prioritization & 86.75\% & 49.40\% & 53.20\% & 00.71\% & 63.16\% \\
ICD & 93.24\% & 68.75\% & 67.52\% & 02.14\% & 76.52\% \\
Paraphrase & 72.74\% & 35.74\% & 32.32\% & 01.80\% & 46.96\% \\
Parden & 74.85\% & 23.40\% & 18.00\% & 04.00\% & 38.75\% \\
Prompt Guard & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
Robust Aligned & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
SafeDecoding & 93.89\% & 67.32\% & 64.52\% & 03.37\% & 75.21\% \\
Self Eval & 95.58\% & 66.84\% & 70.04\% & 05.73\% & 77.51\% \\
Self Reminder & 90.14\% & 69.08\% & 66.51\% & 00.54\% & 75.27\% \\
SmoothLLM & 87.30\% & 56.84\% & 55.76\% & 03.24\% & 66.63\% \\
JBShield & 43.85\% & 25.20\% & 27.56\% & 00.05\% & 32.20\% \\
RPO & 64.60\% & 46.34\% & 46.92\% & 01.81\% & 52.66\% \\
Intention Analysis & 84.44\% & 60.68\% & 62.28\% & 01.05\% & 69.15\% \\
SafeProbing & 94.67\% & 65.88\% & 63.28\% & 04.51\% & 74.61\% \\

\bottomrule
\end{tabular}
\end{table*}





\begin{table*}[t]
\centering
\caption{Attack Success Rate (ASR) of nine jailbreak attacks against representative jailbreak defense methods using the Llama-3.1-8B-Instruct final model. Lower ASR indicates stronger defense robustness.}
\label{tab:asr_attacks_llama}

\scriptsize
\setlength{\tabcolsep}{3.2pt}
\renewcommand{\arraystretch}{1.15}

\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\textbf{Method} &
\textbf{AutoDAN} &
\textbf{PAIR} &
\textbf{TAP} &
\textbf{GCG} &
\textbf{Cipher} &
\textbf{DeepInception} &
\textbf{CodeChameleon} &
\textbf{ICA} &
\textbf{Jailbroken} &
\textbf{Avg. ASR $\downarrow$} \\
\midrule

Vanilla              & 76.00\% & 22.00\% & 40.00\% & 0.00\% & 40.00\% & 42.00\% & 62.00\% & 2.00\% & 22.00\% & 34.00\% \\
Aligner              & 2.00\% & 08.00\% & 8.00\% & 0.00\% & 0.00\% & 4.00\% & 8.00\% & 00.00\% & 8.00\% & 4.22\% \\
Erase and Check      & 46.00\% & 28.00\% & 44.00\% & 0.00\% & 0.00\% & 32.00\% & 18.00\% & 00.00\% & 22.00\% & 21.11\% \\
Goal Prioritization  & 10.00\% & 8.00\% & 14.00\% & 0.00\% & 0.00\% & 12.00\% & 4.00\% & 00.00\% & 8.00\% & 6.22\% \\
ICD                  & 66.00\% & 20.00\% & 24.00\% & 0.00\% & 0.00\% & 16.00\% & 46.00\% & 0.00\% & 10.00\% & 20.22\% \\
Paraphrase           & 0.00\% & 2.00\% & 2.00\% & 0.00\% & 2.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.67\% \\
Parden               & 0.00\% & 16.00\% & 16.00\% & 0.00\% & 0.00\% & 0.00\% & 4.00\% & 0.00\% & 12.00\% &  5.33\% \\
Prompt Guard         & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% \\
Robust Aligned       & 0.00\% & 12.00\% & 16.00\% & 0.00\% & 0.00\% & 8.00\% & 24.00\% & 0.00\% & 0.00\% & 6.67\% \\
SafeDecoding         & 28.00\% & 16.00\% & 24.00\% & 0.00\% & 0.00\% & 44.00\% & 40.00\% & 0.00\% & 6.00\% & 17.56\% \\
Self Eval            & 44.00\% & 10.00\% & 38.00\% & 0.00\% & 0.00\% & 26.00\% & 22.00\% & 0.00\% & 20.0\% & 17.78\% \\
Self Reminder        & 20.00\% & 6.00\% & 6.00\% & 0.00\% & 0.00\% & 8.00\% & 18.00\% & 0.00\% & 0.00\% & 6.44\%  \\
SmoothLLM            & 48.00\% & 20.00\% & 26.00\% & 2.00\% & 6.00\% & 6.00\% & 60.00\% & 0.00\% & 12.00\% & 0.00\% \\
JBShield             & 0.00\% & 6.00\% & 6.00\% &  0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% & 1.33\%  \\
RPO                  & 64.00\% & 02.00\% & 16.00\% & 0.00\% & 0.00\% & 0.00\% & 0.00\% &  0.00\% & 8.00\% & 10.00\% \\
Intention Analysis   & 0.00\% & 4.00\% & 16.00\% & 0.00\% & 0.00\% & 0.00\% & 16.00\% & 0.00\% & 2.00\% & 4.22\% \\
SafeProbing          & 12.00\% & 8.00\% & 18.00\% & 0.00\% & 0.00\% & 2.00\% & 4.00\$ & 0.00\% & 2.00\% & 5.11\% \\

\bottomrule
\end{tabular}
}

\end{table*}



\begin{table*}[t]
\centering
\caption{Attack success rate (ASR) of jailbreak attacks against representative defense methods. Tool model: Qwen3.5-4B; final model: Llama-3.1-8B-Instruct; dataset: AdvBench.}
\label{tab:agentic_attack_defense}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc}
\hline
\textbf{Defense Method} &
\textbf{MINJA ASR (\%)} &
\textbf{TRACE ASR (\%)} &
\textbf{AGENTICRED ASR (\%)} \\
\hline

% Vanilla (No Defense) &  &  &  \\

Self-Evaluation      & 0.00\% & 0.00\% & 2.00\% \\

Self-Reminder        & 0.00\% & 0.00\% & 0.00\% \\

ICD  & 0.00\% & 40.00\% & 2.00\%  \\

Erase and check   & 0.00\% & 0.00\% & 0.00\% \\

Aligner          & 0.00\% & 16.00\% & 4.00\% \\

\hline
\end{tabular}
}
\end{table*}



\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{security_utility_heatmap.pdf}
    \caption{Security vs utility comparison of representative jailbreak defenses. Darker green indicates better performance.}
    \label{fig:security_utility}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{utility_efficiency_heatmap.pdf}
    \caption{Utility vs efficiency comparison of representative jailbreak defenses. Darker green indicates better performance.}
    \label{fig:utility_efficiency}
\end{figure*}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{security_utility_efficiency_heatmap.pdf}
    \caption{Overall comparison of representative jailbreak defenses considering security, utility, and efficiency simultaneously. Darker green indicates better  performance.}
    \label{fig:overall_ranking}
\end{figure*}
